STAR: Statistical Tests with Auditable Results

We present STAR: a novel system aimed at solving the complex issue of "p-hacking" and false discoveries in scientific studies. STAR provides a concrete way for ensuring the application of false discovery control procedures in hypothesis testing, using mathematically provable guarantees, with the goal of reducing the risk of data dredging. STAR generates an efficiently auditable certificate which attests to the validity of each statistical test performed on a dataset. STAR achieves this by using several cryptographic techniques which are combined specifically for this purpose. Under-the-hood, STAR uses a decentralized set of authorities (e.g., research institutions), secure computation techniques, and an append-only ledger which together enable auditing of scientific claims by 3rd parties and matches real world trust assumptions. We implement and evaluate a construction of STAR using the Microsoft SEAL encryption library and SPDZ multi-party computation protocol. Our experimental evaluation demonstrates the practicality of STAR in multiple real world scenarios as a system for certifying scientific discoveries in a tamper-proof way.

==> prelim.tex <==

%\subsection{Homomorphic and Theshold Encryption}
%\label{sec:homomorphicandthreshold}
%\paragraph*{Homomorphic Encryption}
%On primary importance to this work is the ability to compute over encrypted data.
%Homomorphic encryption is a special form of encryption scheme which allows
%manipulating encrypted values without knowledge of the secret key used to encrypt it. 
%This type of encryption
%is useful for evaluating functions privately, i.e., without revealing the inputs
%nor the outputs of the function being evaluated. 



% Commented out by Olya on 06292018
%\paragraph*{Threshold Encryption} 
%One of the main goals of \name is to distribute the power of the data owner to a set
%of computing parties $\partyset$. Thus, it is necessary to distribute the means of 
%decrypting the dataset (i.e., the secret key) to the computing parties in such a way
%that no individual party can decrypt on its own. 
%A threshold-encryption encryption scheme allows for decryption of ciphertexts only 
%when a certain threshold of parties cooperate in the decryption %procedure~\cite{damgaard2010generalization}.
%Specifically, no subset of
%parties smaller than the specified threshold 
%can learn any information, even if they collude amongst %themselves~\cite{damgaard2010generalization}. In essence, this allows us to 
%distribute the ability of the data owner to decrypt the dataset to a set of parties 
%provided that the \emph{majority} of parties are honest with their intentions.



\iflongversion
We summarize the main results for the convenience of the reader. 

The threshold-\paillier encryption scheme is defined as follows:

Let $\partyset$ be a set of $\np$ parties (decryption servers) where a threshold of $t \leq \np$ are required to participate in order to decrypt a ciphertext.

\paragraph*{Key Generation}
\label{sec:paillierkeygen}
Pick two $N$-bit primes, $p$ and $q$ such that $p = 2p' + 1$ and $q = 2q' + 1$ where $p',q'$ are Sophie Germain primes. \\
Set $N = pq$ and $M = p'q'$.\\
Let $\lambda = lcm(p-1, q-1)$
and let the master secret key $\pailliersk = \lambda$. 
Pick an integer $d$ such that $d \equiv 1 \nspmod{N^2}$ and $d \equiv 0 \nspmod{M}$\footnote{\cite{damgaard2010generalization} warns the reader that using $d=\lambda$ (as per the original \paillier scheme) is not secure in the threshold setting. Therefore, $d$ must be chosen independently of $\lambda$.}\\
Set $t$ such that $2t - 1 \leq \np$ and construct the polynomial $f(X) = \sum_{i = 0}^{t-1} a_iX^i \nspmod{N^2M}$ where $a_i$ for $i \ge 1$ is picked at random from the set $ \{0,1,\dots,N^2M-1\}$. Set $a_0 = d$. For $i = 1\dots \np$, $\player_i$ receives the secret share $s_i = f(i)$ of the secret key $\pailliersk$. \\
Set the public key $\paillierpk = N$. For verification of each party's actions during the decryption phase, pick a public generator $v$ for the cyclic group of quadratic residues in $\Z_{N^2}^*$. For $i = 1\dots \np$, $\player_i$ gets the verification key $v_i = v^{s_i\Delta} \nspmod{N^2}$ where $\Delta = \np!$.


\paragraph*{Encryption}
To encrypt a message $m \in Z_{N}$,
pick a random $r \in \Z_{N^2}$ and compute the ciphertext $c = (N+1)^mr^{N^2} \pmod{N^2}$. 

\paragraph*{Homomorphic Addition}
Addition of two ciphertexts $c_1, c_2 \in Z_{N^2}$ is computed as follows:
pick a random $r \in \Z_{N^2}$ and compute $c' = (c_1c_2)r^{N^2} \nspmod{N^2}$. Observe that $c_1c_2 = (N+1)^{m_1 + m_2}(r')^{N^2}$ for some $r' \in \Z_{N^2}$ hence the result is correct. We note that the randomization step may be omitted when deterministic computations are acceptable or required. 

\paragraph*{Homomorphic Multiplication}
Multiplication of a ciphertext $c \in Z_{N^2}$ by a public constant $s \in Z_N$ is computed as follows:
pick a random $r \in \Z_{N^2}$ and compute $c' = c_1^sr^{N^2} \nspmod{N^2}$. Observe that $c_1^s = (n+1)^{m_1s}(r')^{N^2}$ for some $r' \in \Z_{N^2}$ hence the result is correct. Once more, the randomization step may be omitted if needed. 


\paragraph*{Threshold Decryption}

To decrypt a ciphertext $c$, each
player $\player_i \in \partyset$ computes $c_i = c^{2\Delta s_i}$ where $\Delta = \np!$ and $s_i$ is the secret share of the secret key $\pailliersk$ held by $\player_i$. Additionally, $\player_i$ produces a zero-knowledge proof that $\log_{c^4}(c^2_i) = \log_{v}(v_i)$ which will prove that $\player_i$ indeed raised the ciphertext $c$ to the private exponent $s_i$. Such a non-interactive zero-knowledge proof can be derived using the Fiat-Shamir heuristic described in \cite{shoup2000practical,damgaard2010generalization}.   

With the required $t$ unique shares $(c_1,\dots, c_t)$ with the corresponding zero-knowledge proofs of correctness, the decryption can be computed by taking the set $S = \{c_1,\dots, c_t\}$ of $t$ shares and combining them using Lagrange interpolation as follows:
\[
c' = \prod_{i \in S}^{} c_{i}^{2\lambda_{0,i}^S} \text{ where } \lambda_{0,i}^S = \Delta \prod_{i' \in S\setminus \{i\}}^{} \frac{i}{i' - i} \in \Z
\]
Note that $c' = c^{4\Delta^2f(0)} = c^{4\Delta^2d}$. Since $4\Delta^2d \equiv 0 \nspmod{\lambda}$ and $4\Delta^2d \equiv 4\Delta^2d \nspmod{N^2}$, we get that $c' = (n + 1)^{4\Delta^2 m}$ where $m$ is the plaintext we wish to extract. Therefore, $4\Delta^2m$ can be efficiently obtained as described in the original \paillier which allows us to recover $m$ as follows:
\[
m = L(c' \nsmod {N^2}) (4\Delta^2)^{-1} \nspmod{N}
\]
where $L(u) = \frac{u-1}{N}$ as specified in \cite{paillier1999public,damgaard2010generalization}.  
\fi



%A blockchain is a decentralized storage mechanism for recording transactions that guarantees data (state) immutability
%while being maintained by many nodes  through a distributed cryptographic protocol~\cite{cachin2017blockchains}. 
%All nodes validate the information to be appended to the blockchain and use a consensus protocol to ensure that the nodes agree on a unique order in which entries are appended.
%First described as a building block for the Bitcoin cryptocurrency \cite{nakamoto2008bitcoin}, blockchains have
%gained popularity as a multi-purpose distributed ledger mechanism with broad applications.
%In general, a blockchain 
%is a series of \new{blocks}, each containing a set of \emph{transactions}. Each block is cryptographically linked to previous blocks in a \new{chain} and stored by each peer in a set of peers participating the protocol. Assuming an honest majority of peers correctly following the protocol, the chain of blocks is guaranteed to be correct and immutable. 
%
%In this work, we require a permissioned blockchain that is world-readable (i.e., public) but is restricted when it comes to 
%adding transactions (i.e., only a subset of nodes have write privileges). Such a construction is described in \cite{zyskind2015decentralizing} and expanded on in \cite{zyskind2016efficient}. We require that a trusted
%authority (in our case, the data owner) approve a set
%of parties for write access.
%\fixme{Such a construction can easily be expanded to a trustless setting using SMPC where
%a threshold majority is required to bestow write access to a new peer.}
%
%We abstract out the actual implementation of the blockchain (e.g., the consensus protocol or expressiveness
%of the language).
%\fixme{add an ideal functionality of a permissioned blockchain. e.g., one that takes party identifiers
%	and provides access to read index, write (index, data) to them}



%
%Of importance to this work is that statistically secure protocols are secure when composed with other statistically and perfectly secure protocols\cite{bogdanov2014input}. We use this fact when proving security of protocols presented in this paper. 


\iflongversion

A summary of notation used throughout this work is listen in Table \ref{table:notation}.
\begin{table}[h]\caption{Summary of Notation}
	\centering % to have the caption near the table
	\begin{tabular}{l c p{6.8cm} }
		\toprule
		\arrayrulecolor{black! 10}
		$\owner$ & $\space$ & Owner of a dataset and the master keys used to encrypt it.\\
		\midrule
		$\np$ & $\space$ & Number of computing parties.\\
		\midrule
		$t$ & $\space$ & Thrshold number of parties required to reveal (or decrypt) a secret share.\\
		\midrule
		$\player_i$ & $\space$ & Computing party from the set of parties $\partyset$.\\
		\midrule		
		$\bl$ & $\space$ & Number of bits required to represent the largest integer during a computation.\\
		\midrule
		$\fpparam$ & $\space$ & Number of bits of precision required for fixed-point arithmetic computations.\\
		\midrule
		$\kappa$ & $\space$ & Statistical security parameter for statistically private protocols.\\
		\arrayrulecolor{black! 10}\midrule
		$\share{s}$ & $\space$ & Secret share (or encryption) of the a secret integer $s$.\\
		\midrule
		$\bshare{s}$ & $\space$ & Secret shares (or encryptions) of the bitwise representation of a secret integer $s$.\\
		\midrule	
		$\Ds$ & $\space$ & A dataset containing containing rows and columns where each cell contains a value from $\R$.\\
		\midrule
		$\dshare{\Ds}{}$ &$\space$ & Secret share (or encryption) of the dataset $\Ds$. Each cell of 
		$\Ds$ is a secret share (or encryption) of the fixed-point representation of the real value found in that cell.\\
		\midrule
		$\dsize$ & $\space$ & Number of rows in the dataset $\Ds$.\\
		\midrule
		$\attr{i}$ & $\space$ & The $i$th attribute (column) in the dataset $\Ds$.\\
		\arrayrulecolor{black!}
		\bottomrule
	\end{tabular}
	\label{table:notation}
\end{table}
\fi
